Program Analysis of Probabilistic Programs

Probabilistic programming is a growing area that strives to make statistical analysis more accessible, by separating probabilistic modelling from probabilistic inference. In practice this decoupling is difficult. No single inference algorithm can be used as a probabilistic programming back-end that is simultaneously reliable, efficient, black-box, and general. Probabilistic programming languages often choose a single algorithm to apply to a given problem, thus inheriting its limitations. While substantial work has been done both to formalise probabilistic programming and to improve efficiency of inference, there has been little work that makes use of the available program structure, by formally analysing it, to better utilise the underlying inference algorithm. This dissertation presents three novel techniques (both static and dynamic), which aim to improve probabilistic programming using program analysis. The techniques analyse a probabilistic program and adapt it to make inference more efficient, sometimes in a way that would have been tedious or impossible to do by hand.

==> toc.tex <==
\chapter*{\sc Table of Contents}
\contentsline {chapter}{\numberline {1}Introduction}{1}{chapter.1}%
\contentsline {chapter}{\numberline {2}Probabilistic programming}{5}{chapter.2}%
\contentsline {section}{\numberline {2.1}A very simple probabilistic program}{5}{section.2.1}%
\contentsline {paragraph}{Notation and terminology}{6}{paragraph*.2}%
\contentsline {section}{\numberline {2.2}Bayesian inference}{7}{section.2.2}%
\contentsline {subsection}{\numberline {2.2.1}Deriving a solution analytically}{7}{subsection.2.2.1}%
\contentsline {subsection}{\numberline {2.2.2}Rejection sampling and the curse of dimensionality}{7}{subsection.2.2.2}%
\contentsline {subsection}{\numberline {2.2.3}Markov chain Monte Carlo inference}{9}{subsection.2.2.3}%
\contentsline {subsection}{\numberline {2.2.4}Variational inference}{13}{subsection.2.2.4}%
\contentsline {subsection}{\numberline {2.2.5}Inference on graphical models}{16}{subsection.2.2.5}%
\contentsline {subsection}{\numberline {2.2.6}Other inference strategies}{20}{subsection.2.2.6}%
\contentsline {section}{\numberline {2.3}Probabilistic programming languages}{22}{section.2.3}%
\contentsline {subsection}{\numberline {2.3.1}Definition and classification of PPLs}{22}{subsection.2.3.1}%
\contentsline {subsection}{\numberline {2.3.2}Density-based (or \textit {explicit}) PPLs}{24}{subsection.2.3.2}%
\contentsline {subparagraph}{Inference.}{26}{subparagraph*.10}%
\contentsline {subparagraph}{Strengths.}{26}{subparagraph*.11}%
\contentsline {subparagraph}{Constraints.}{27}{subparagraph*.12}%
\contentsline {subparagraph}{Inference.}{27}{subparagraph*.13}%
\contentsline {subparagraph}{Strengths:}{28}{subparagraph*.14}%
\contentsline {subparagraph}{Constraints:}{28}{subparagraph*.15}%
\contentsline {subsection}{\numberline {2.3.3}Sample-based (or \textit {implicit}) PPLs}{28}{subsection.2.3.3}%
\contentsline {subparagraph}{Inference:}{29}{subparagraph*.17}%
\contentsline {subparagraph}{Strengths:}{30}{subparagraph*.18}%
\contentsline {subparagraph}{Constraints:}{30}{subparagraph*.19}%
\contentsline {subparagraph}{Inference:}{30}{subparagraph*.21}%
\contentsline {subparagraph}{Strengths:}{31}{subparagraph*.22}%
\contentsline {subparagraph}{Constraints:}{31}{subparagraph*.23}%
\contentsline {subsection}{\numberline {2.3.4}Effect-handling-based PPLs}{31}{subsection.2.3.4}%
\contentsline {subparagraph}{Inference:}{33}{subparagraph*.24}%
\contentsline {subparagraph}{Strengths:}{33}{subparagraph*.25}%
\contentsline {subparagraph}{Constraints:}{33}{subparagraph*.26}%
\contentsline {part}{I\hspace {1em}Static optimisation for probabilistic programming}{35}{part.1}%
\contentsline {chapter}{\numberline {3}Formal treatment of programming languages}{37}{chapter.3}%
\contentsline {section}{\numberline {3.1}Formal syntax of programming languages}{37}{section.3.1}%
\contentsline {section}{\numberline {3.2}Rules of inference}{38}{section.3.2}%
\contentsline {section}{\numberline {3.3}Semantics of programming languages}{40}{section.3.3}%
\contentsline {section}{\numberline {3.4}Type checking and type inference}{41}{section.3.4}%
\contentsline {section}{\numberline {3.5}Information flow analysis}{42}{section.3.5}%
\contentsline {chapter}{\numberline {4}SlicStan}{45}{chapter.4}%
\contentsline {section}{\numberline {4.1}The paper}{45}{section.4.1}%
\contentsline {subsection}{\ignorespaces 1 Introduction}{46}{subsection.4.1.1}%
\contentsline {subsubsection}{\ignorespaces 1.1 Background: Probabilistic Programming Languages and Stan}{46}{subsubsection.4.1.1.1}%
\contentsline {subsubsection}{\ignorespaces 1.2 Goals and Key Insight}{47}{subsubsection.4.1.1.2}%
\contentsline {subsubsection}{\ignorespaces 1.3 The Insight by Example}{47}{subsubsection.4.1.1.3}%
\contentsline {subsubsection}{\ignorespaces 1.4 Core Contributions and Outline}{48}{subsubsection.4.1.1.4}%
\contentsline {subsection}{\ignorespaces 2 Core Stan}{48}{subsection.4.1.2}%
\contentsline {subsubsection}{\ignorespaces 2.1 Syntax of Core Stan Expressions and Statements}{48}{subsubsection.4.1.2.1}%
\contentsline {subsubsection}{\ignorespaces 2.2 Operational Semantics of Stan Statements}{49}{subsubsection.4.1.2.2}%
\contentsline {subsubsection}{\ignorespaces 2.3 Syntax of Stan}{50}{subsubsection.4.1.2.3}%
\contentsline {subsubsection}{\ignorespaces 2.4 Density-Based Semantics of Stan}{51}{subsubsection.4.1.2.4}%
\contentsline {subsubsection}{\ignorespaces 2.5 Inference}{53}{subsubsection.4.1.2.5}%
\contentsline {subsection}{\ignorespaces 3 SlicStan}{53}{subsection.4.1.3}%
\contentsline {subsubsection}{\ignorespaces 3.1 Syntax}{54}{subsubsection.4.1.3.1}%
\contentsline {subsubsection}{\ignorespaces 3.2 Typing of SlicStan}{55}{subsubsection.4.1.3.2}%
\contentsline {subsubsection}{\ignorespaces 3.3 Elaboration of SlicStan}{58}{subsubsection.4.1.3.3}%
\contentsline {subsubsection}{\ignorespaces 3.4 Semantics of SlicStan}{60}{subsubsection.4.1.3.4}%
\contentsline {subsubsection}{\ignorespaces 3.5 Examples}{60}{subsubsection.4.1.3.5}%
\contentsline {subsubsection}{\ignorespaces 3.6 Difficulty of Specifying Direct Semantics Without Elaboration}{62}{subsubsection.4.1.3.6}%
\contentsline {section}{\numberline {4.2}Clarifying the contributions}{94}{section.4.2}%
\contentsline {paragraph}{Author contributions.}{94}{paragraph*.27}%
\contentsline {paragraph}{Similarities to previous work.}{94}{paragraph*.28}%
\contentsline {paragraph}{Contributions of this chapter.}{94}{paragraph*.29}%
\contentsline {section}{\numberline {4.3}Impact}{96}{section.4.3}%
\contentsline {chapter}{\numberline {5}Conditional independence by typing}{97}{chapter.5}%
\contentsline {section}{\numberline {5.1}The paper}{97}{section.5.1}%
\contentsline {paragraph}{Author contributions.}{98}{paragraph*.30}%
\contentsline {section}{\numberline {5.2}Discussion}{153}{section.5.2}%
\contentsline {part}{II\hspace {1em}Dynamic optimisation for probabilistic programming}{155}{part.2}%
\contentsline {chapter}{\numberline {6}Automatic reparameterisation}{157}{chapter.6}%
\contentsline {section}{\numberline {6.1}Effect-handling based probabilistic programming}{157}{section.6.1}%
\contentsline {subsection}{\numberline {6.1.1}Effects and effect handling}{158}{subsection.6.1.1}%
\contentsline {paragraph}{Types of effect handlers.}{159}{paragraph*.31}%
\contentsline {subsection}{\numberline {6.1.2}Composing effect handlers}{159}{subsection.6.1.2}%
\contentsline {subsection}{\numberline {6.1.3}Effect handling in probabilistic programming}{160}{subsection.6.1.3}%
\contentsline {section}{\numberline {6.2}The paper}{162}{section.6.2}%
\contentsline {paragraph}{Author contributions.}{162}{paragraph*.32}%
\contentsline {section}{\numberline {6.3}Discussion}{179}{section.6.3}%
\contentsline {subsection}{\numberline {6.3.1}Impact}{179}{subsection.6.3.1}%
\contentsline {subsection}{\numberline {6.3.2}Scope and extensions}{179}{subsection.6.3.2}%
\contentsline {paragraph}{Multivariate distributions.}{179}{paragraph*.33}%
\contentsline {paragraph}{Other reparameterisations.}{179}{paragraph*.34}%
\vspace \bigskipamount 
\contentsline {chapter}{\numberline {7}Challenges ahead}{181}{chapter.7}%
\contentsline {chapter}{Bibliography}{182}{appendix*.35}%

